Performance comparison of CFD-DEM solver MFiX-Exa, on GPUs and CPUs

We present computational performance comparisons of gas-solid simulations performed on current CPU and GPU architectures using MFiX Exa, a CFD-DEM solver that leverages hybrid CPU+GPU parallelism. A representative fluidized bed simulation with varying particle numbers from 2 to 67 million is used to compare serial and parallel performance. A single GPU was observed to be about 10 times faster compared to a single CPU core. The use of 3 GPUs on a single compute node was observed to be 4x faster than using all 64 CPU cores. We also observed that using an error controlled adaptive time stepping scheme for particle advance provided a consistent 4x speed-up on both CPUs and GPUs. Weak scaling results indicate superior parallel efficiencies when using GPUs compared to CPUs for the problem sizes studied in this work.

==> version2.tex <==
\subsubsection{Array-of-structures vs structure-of-array paradigms}
%
A roofline model can be used indicate when a software module is limited by memory or computation. We compared the performance of MFix-Exa using two types of memory layouts for particle data: Array of Structures (AoS) and Structure of Arrays (SoA). 
Each of the particle parameters (for e.g. velocity, angular velocity, particle drag) are stored within a structure in the AoS format and an array of these structures make up the entire particle data in a simulation.
%In the AoS format each particle's parameter is stored in a structure and the particle array contains an array of these structures. 
In the SoA format, separate arrays with a size equal to the number of particles are used for each particle parameter within a \emph{box}. 
A single core simulation of the fluidized bed case with 160,000 particles was simulated for 10 timesteps. The roofline analysis of this 
simulation is presented in Fig.\ \ref{aos_vs_soa}(a) and (b) where each function in the code is represented as a point in the performance-arithmetic-intensity space. 
%
\begin{figure}
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{figures/aossoa_old_one_grid_larger_font.png}
\caption{}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{figures/aossoa_new_one_grid_larger_font.png}
\caption{}
\end{subfigure}
\caption{Roofline analysis of various functions (represented as green and red dots) for a simulation with 160,000 particles on a single core CPU using (a) AoS and (b) SoA paradigms, respectively. Red dots show functions which take a larger percentage of the total runtime.}
\label{aos_vs_soa}
\end{figure}
%
The SoA paradigm was implemented to optimize performance on the GPU, but it tends to have negative effects on CPU performance. We observed that several functions became more memory bound using the SoA paradigm as can be seen by comparing Fig.\ \ref{aos_vs_soa}(a) and (b). A large cluster of points in the AoS case (Fig.\ \ref{aos_vs_soa}(a)) seems to get spread to the lower left of the roofline plot in Fig.\ \ref{aos_vs_soa}(b) indicating suboptimal performance. The SoA paradigm resulted in 22\% of the code being vectorized as opposed to a considerably lower value of 13\% with the AoS paradigm.
%
